El Agente Cuantico: Automating quantum simulations

Quantum simulation is central to understanding and designing quantum systems across physics and chemistry. Yet it has barriers to access from both computational complexity and computational perspectives, due to the exponential growth of Hilbert space and the complexity of modern software tools. Here we introduce{\cinzel El Agente Cu\'antico}, a multi-agent AI system that automates quantum-simulation workflows by translating natural-language scientific intent into executed and validated computations across heterogeneous quantum-software frameworks. By reasoning directly over library documentation and APIs, our agentic system dynamically assembles end-to-end simulations spanning state preparation, closed- and open-system dynamics, tensor-network methods, quantum control, quantum error correction, and quantum resource estimation. The developed system unifies traditionally distinct simulation paradigms behind a single natural-language interface. Beyond reducing technical barriers, this approach opens a path toward scalable, adaptive, and increasingly autonomous quantum simulation, enabling faster exploration of physical models, rapid hypothesis testing, and closer integration between theory, simulation, and emerging quantum hardware.

==> editing_commands.tex <==
% NOTE:
% All editing commands contain curly braces {} around them so that 
% they can easily be searched for in the final document via cmd + f.

% Highlighted comments for authors
\usepackage{soul, color}
\newcommand{\Note}[1]{}
\renewcommand{\Note}[1]{#1}  % comment out this re-definition to suppress all Notes
\newcommand{\NoteSigned}[3]{{\textcolor{#2}{\Note{\textbf{[#1: #3]}}}}}
% Alternative with highlighter color rather than text colour
%\renewcommand{\NoteSigned}[3]{{\sethlcolor{#2}\Note{\hl{#1: #3}}}}

% Specific author comments
\newcommand{\pl}[1]{\NoteSigned{PL}{blue}{#1}}  % use for notes from Pietro
\newcommand{\tc}[1]{\NoteSigned{TC}{green}{#1}}
\newcommand{\cb}[1]{\NoteSigned{CB}{brown}{#1}}
\newcommand{\cj}[1]{\NoteSigned{CJ}{purple}{#1}}
\newcommand{\sm}[1]{\NoteSigned{SM}{magenta}{#1}}

% Inline todo: Flag something in the text to be done
\newcommand{\itodo}[1]{\NoteSigned{TODO}{red}{#1}}
% Preliminary: Flag preliminary statements or results
\newcommand{\prelim}[1]{\NoteSigned{Prelim}{grey}{#1}}

% Convenient other commands
\newcommand{\sowhat}{$\rightarrow$~}


% Variant of the TODO box for addressing reviewer comments
\newcommand{\bluebox}[1]{\todo[color=blue!20!white]{#1}}

